Extrapolating gravitational-wave data from numerical simulations

Two complementary techniques are developed for obtaining the asymptotic form of gravitational-wave data at large radii from numerical simulations, in the form of easily implemented algorithms. It is shown that, without extrapolation, near-field effects produce errors in extracted waveforms that can significantly affect LIGO data analysis. The extrapolation techniques are discussed in the context of Newman--Penrose data applied to extrapolation of waveforms from an equal-mass, nonspinning black-hole binary simulation. The results of the two methods are shown to agree within error estimates. The various benefits and deficiencies of the methods are discussed.

==> Preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is all for the hyperref package, and nice colors
\RequirePackage{ifpdf}
\ifpdf
%\usepackage{pdfsync}
%\usepackage{thumbpdf}
\usepackage[backref=page, colorlinks, hyperfootnotes=false, %
plainpages=false, bookmarksnumbered, pdfpagemode=UseNone, %
hyperfigures=true]{hyperref}
\else
\usepackage[backref=page, colorlinks, pdfborder={0 0 0}, hyperindex,%
plainpages=false]{hyperref}
\fi
\renewcommand*{\backref}[1]{}
\renewcommand*{\backrefalt}[4]{% 
  \ifcase #1 { } \or (Cited on page~#2.) \else %
  (Cited on pages~#2.) \fi %
}
\definecolor{ChapterColor}{rgb}{0.510, 0.118, 0.000}
\definecolor{LinkColor}   {rgb}{0.741, 0.173, 0.000}
\definecolor{CiteColor}   {rgb}{0.000, 0.502, 0.118}
\definecolor{UrlColor}    {rgb}{0.000, 0.212, 0.800}
\hypersetup{linkcolor=LinkColor}
\hypersetup{citecolor=CiteColor}
\hypersetup{urlcolor=UrlColor}
%\hypersetup{pdflang={English}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

